Adaptive Weight Learning for Multiple Outcome Optimization With Continuous Treatment

To promote precision medicine, individualized treatment regimes (ITRs) are crucial for optimizing the expected clinical outcome based on patient-specific characteristics. However, existing ITR research has primarily focused on scenarios with categorical treatment options and a single outcome. In reality, clinicians often encounter scenarios with continuous treatment options and multiple, potentially competing outcomes, such as medicine efficacy and unavoidable toxicity. To balance these outcomes, a proper weight is necessary, which should be learned in a data-driven manner that considers both patient preference and clinician expertise. In this paper, we present a novel algorithm for developing individualized treatment regimes (ITRs) that incorporate continuous treatment options and multiple outcomes, utilizing observational data. Our approach assumes that clinicians are optimizing individualized patient utilities with sub-optimal treatment decisions that are at least better than random assignment. Treatment assignment is assumed to directly depend on the true underlying utility of the treatment rather than patient characteristics. The proposed method simultaneously estimates the weighting of composite outcomes and the decision-making process, allowing for construction of individualized treatment regimes with continuous doses. The proposed estimators can be used for inference and variable selection, facilitating the identification of informative treatment assignments and preference-associated variables. We evaluate the finite sample performance of our proposed method via simulation studies and apply it to a real data application of radiation oncology analysis.

==> table.tex <==


\begin{table}[h]
\caption{Condition with continuous optimal treatment: n = 500, p = 50, $E(Y(g_{opt}))=10${;} reported values are based on 100 Monte Carlo replications, using a test set of size 10000.}
\begin{tabular}{>{\sf }llllllll} %
\cmidrule{1-8}

Model  &$E(Y(\hat{g}_{opt}))$ & RMSE of $\hat{g}_{opt}$ & Tree Height\\
\midrule
GoDoTreep10 & 7.795 (0.19) & 0.125 (0.01) & 2 \\
GoDoTree & 8.19 (0.23) & 0.112 (0.01) & 3 \\
CART & 7.78 (0.19) & 0.136 (0.01) & 2 \\
CART & 7.93 (0.20) & 0.128 (0.01) & 3 \\
LZ   &  7.93 (0.27)& 0.125 (0.01)  &2  \\
LZ   &  8.10 (0.23)&  0.118 (0.01)  &3  \\
Random & 5.49 (0.09) & 0.353 (0.01) & NA \\

%GoDoTreep50 & 7.73 (0.25) & 0.138 (0.01) & 2 \\
GoDoTree & 7.94 (0.29) & 0.127 (0.02) & 3 \\
%CART & 7.68 (0.19) & 0.140 (0.01) & 2 \\
CART & 7.74 (0.23) & 0.142 (0.01) & 3 \\
LZ   & 7.88 (0.25) & 0.128 (0.01) & 2 \\
LZ   & 7.88 (0.24) & 0.133 (0.02) & 3 \\
Random & 5.48 (0.10) & 0.353 (0.01) & NA \\

\bottomrule
\end{tabular}
\end{table}	



\begin{table}[h]
\caption{Condition when greedy search can not achieve global optimum: n = 500, p = 10, $E(Y(g_{opt}))=10${;} reported values are based on 100 Monte Carlo replications, using a test set of size 1000.}
\begin{tabular}{>{\sf }lllll} %
\cmidrule{1-5}
Model  &$E(Y(\hat{g}_{opt}))$ & RMSE of $\hat{g}_{opt}$ & Tree Height\\
\midrule
%GoDoTree p10 & 7.49 (1.29) & 0.15 (0.04) & 2 \\
GoDoTree & 7.65 (0.84) & 0.15 (0.02) & 3 \\
%CART & 4.29 (0.71) & 0.24 (0.02) & 2 \\
CART & 4.74 (0.96) & 0.23 (0.02) & 3 \\
LZ       & 3.00 (2.31) & 0.65 (0.04) & 2 \\
LZ       & 2.09 (3.38) & 0.66 (0.04) & 3 \\
Random & -4.55 (0.52) & 0.38 (0.01) & NA \\
%GoDoTree p50 & 5.46 (1.19) & 0.21 (0.03) & 2 \\
GoDoTree & 5.66 (1.05) & 0.21 (0.03) & 3 \\
%CART & 3.76 (0.24) & 0.25 (0.004) & 2 \\
CART & 3.76 (0.27) & 0.25 (0.005) & 3 \\
LZ      &-0.95 (1.85) & 0.66 (0.04)   & 2 \\
LZ      &1.57 (1.45) & 0.67 (0.05)   & 3 \\
Random & -4.53 (0.54) & 0.38 (0.01) & NA \\

\bottomrule
\end{tabular}
\end{table}	





optimize its parameter $\eta = (j,b,sign)$, where $j$ is $j^{th}$ variable to be used as the classifier, $b$ is corresponding split rule and $\text{sign} \in \{1,-1\}$ is the sign indicator. Then this node represent a partition $\delta_{\eta}$ that divide $\mathscr{S}$ into two parts:

\begin{equation*}
    \delta_{\eta}(\bold{X}) = \left\{
    \begin{aligned}
        &left&,  (z_j-b)\times sign < 0\\
        &right&, (z_j-b) \times sign \geq 0\\
    \end{aligned}
    \right.
\end{equation*}

where $z_j$ is $j$ th variable of $\bold{X}$.










\iffalse

\begin{algorithm}
\caption{Put your caption here}
\begin{algorithmic}[1]
    \State Initialize a regression tree with height h, set t=0
    \While{not converge} 
    \For{\texttt{i in 1 to h}}    \Comment{Forward optimization}
        \For{\texttt{every node in height i}}
            \State Denote $\eta_0$ as current parameter
            \State Draw a random variable and splitting rule $\eta_i$ as a new predictor
            \State Calculate $W(\eta_0)$ and W($\eta_i$)
            \If{ $W(\eta_i) \geq W(\eta_0)$ }
                \State Update node parameter $\eta$ with $\eta_i$ 
            \ElsIf{$W(\eta_i) < W(\eta_0)$}
                \State Update node parameter $\eta$ with probability $P(\eta = \eta_j) = \frac{exp( \alpha_t (W(\eta_i)))}{exp( \alpha_t (W(\eta_0)))}  $ 
            \EndIf
        \If{ one child is empty }
            \State replace the node with non-empty child 
        \EndIf
        \EndFor
    \EndFor
    
    \For{\texttt{every leaf node}}
        \State \texttt{find the best prediction}
    \EndFor
    
    \For{\texttt{i in h to 1}}    \Comment{Forward optimization}
        \For{\texttt{every node in height i}}
            \State Denote $\eta_0$ as current parameter
            \State Draw a random variable and splitting rule $\eta_i$ as a new predictor
            \State Calculate $W(\eta_0)$ and W($\eta_i$)
            \If{ $W(\eta_i) \geq W(\eta_0)$ }
                \State Update node parameter $\eta$ with $\eta_i$ 
            \ElsIf{$W(\eta_i) < W(\eta_0)$}
                \State Update node parameter $\eta$ with probability $P(\eta = \eta_j) = \frac{exp( \alpha_t (W(\eta_i)))}{exp( \alpha_t (W(\eta_0)))}  $ 
            \EndIf
        \If{ one child is empty }
            \State replace the node with non-empty child 
        \EndIf
        \EndFor
    \EndFor
    \State t = t+1
    
    \EndWhile\label{euclidendwhile}

\end{algorithmic}
\end{algorithm}

\fi


==> theorem.tex <==

Regular effect curve $\theta(a)$ can be identified with observed data as 
\begin{equation}
    \theta(a) = \mathbb{E} Y^a  = \mathbb{E} \{ \mu(\bold{L},a) \} = 
    \int_{\mathscr{L}} \mu(\bold{l},a) dP(\bold{l})
\end{equation}

But since we are considering the personalized effect curve, our parameter of interest change into  

\begin{equation}
    \theta_l(a) = \mathbb{E} Y^{a,l} = \mu(l,a) 
    \frac{\int_{\mathscr{L}} \mu(\bold{x},a)K_{bl}(\bold{x})  dP(\bold{x})}{\int_{\mathscr{L}} K_{bl}( \bold{x})  dP(\bold{x})} =  \frac{ \mathbb{E} \mu(\bold{X},a)K_{bl}(\bold{X}) }{\mathbb{E} K_{bl}( \bold{X})} 
\end{equation}

where $K_{bl}(\bold{x}) = b^{-1} K\{ (x - l)/b \}$ with $K$ a standard kernal function (a symmetric probability density) and b a scalar bandwidth parameter.

Although $\mu(l,a)$ can be estiamted straightforwardly,  we aimed to find its doubly robust estimate $\xi(\bold{Z};\hat{\pi},\hat{\mu})$ of the observed data $\bold{Z}$ and nuisance functions $(\pi,\mu)$ such that $\mathbb{E} (\xi(A;\bar{\pi},\bar{\mu})\mid A=a) = \theta(a)$, if either $\bar{\pi} = \pi$ or $\bar{\mu} = \mu$ (not necessarily both).
  

To derive doubly robust estimators for θ(a) without relying on parametric models, we adapt semiparametric theory in a novel way similar to the approach of Rubin and van der Laan (2005, 2006a). Specifically, if $\mathbb{E} (\xi(A;\bar{\pi},\bar{\mu})\mid A=a) = \theta(a)$ then it follows that $\mathbb{E} (\xi(A;\bar{\pi},\bar{\mu})) = \psi$ for 
\begin{equation}
    \psi = \mathbb{E} \theta_l(a)  =   \int_{\mathscr{A}} \theta_l(a)w(a) da
\end{equation}




Theorem 1:

Under a nonparametric model, the efficient influence function for $\psi = \int_{\mathscr{A}} \theta_l(a)w(a) da$ is 

$$\xi - \psi + (\mathbb{E} K_{bl}(\bold{X}))^{-1} \int_{\mathscr{A}} [\mu(\bold{X},a)K_{bl}(\bold{X}) - m(a)]w(a)da $$

$$\xi(\bold{Z};\pi,\mu) = (\mathbb{E} K_{bl}(\bold{X}))^{-1}
[\frac{Y-\mu(\bold{X},A)}{\pi(A\mid \bold{X})}w(A)K_{bl}(\bold{X}) + m(A)]
 $$

where $w(a) = \int_{}\pi(a\mid x)dP(x) = \mathbb{E} \pi(a\mid \bold{X})$ and $m(a) = \int_{}\mu(x,a ) K_{bl}(\bold{x}) dP(x) = \mathbb{E} \mu(\bold{X},a ) K_{bl}(\bold{X}) $.

Proof：

$$\phi(\bold{Z}) = (\mathbb{E} K_{bl}(\bold{X}))^{-1}
\{ \frac{Y-\mu(\bold{X},A)}{\pi(A\mid \bold{X})}w(A)K_{bl}(\bold{X}) + m(A) +  \int_{\mathscr{A}} [\mu(\bold{X},a)K_{bl}(\bold{X}) - m(a)]w(a)da \} - \psi$$



Let $p(\bold{z};\epsilon)$ be a parametric submodel with parameter $\epsilon \in \mathbb{R}$ and $p(\bold{z};0) = p(\bold{z})$, for example $p(\bold{z};\epsilon) = \{1+\epsilon b(\bold{z}) \} p(\bold{z})$ where $\mathbb{E} \{b(\bold{Z})\} = 0$ with $\lvert b(\bold{z})\lvert <B$ and $\lvert  \epsilon \lvert  < 1/B$ to ensure that $p(\bold{z};\epsilon) \ge 0$. For notational simplicity we denote $\{ \partial f(\bold{t};\epsilon) / \partial \epsilon \}\mid_{\eplison = 0}$ by $f'_{\epsilon}(\bold{t};0)$ for any general function $f$ of $\epsilon$ and other arguments $\bold{t}$.

By definition the efficient influence function for $\psi$ is the unique function $\phi(\bold{Z})$ that satisfies $\psi'_{\epsilon}(0) = \mathbb{E} \{\phi(\bold{Z}) l'_{\epsilon}(\bold{Z};0) \}$, where $\psi(\epsilon)$ represents the parameter of interest as a functional on the parametric submodel and $l(\bold{w} \lvert \bold{ \bar{w}};\epsilon) = log p(\bold{w} \lvert \bold{ \bar{w}};\epsilon)$ for any partition $(\bold{W},\bold{ \bar{W} }) \subset \bold{Z}$. Therefore 

$$ l'_{\epsilon}(\bold{z};\epsilon) = 
l'_{\epsilon}(y \lvert \bold{l},a;\epsilon) + 
l'_{\epsilon}(a \lvert \bold{l};\epsilon) + 
l'_{\epsilon}(\bold{l};\epsilon) $$

We give two two important properties of such score functions $l'_{\epsilon}(\bold{w} \lvert \bold{ \bar{w}};\epsilon)$ that will be use throughout the following proof. 

The first one is that $l'_{\epsilon}(\bold{w} \lvert \bold{ \bar{w}};\epsilon) = p'_{\epsilon}(\bold{w} \lvert \bold{ \bar{w}};\epsilon) / p(\bold{w} \lvert \bold{ \bar{w}};\epsilon)$ because $l(\bold{w} \lvert \bold{ \bar{w}};\epsilon)$ is a log transformation of $p(\bold{w} \lvert \bold{ \bar{w}};\epsilon)$.

Secondly, as with any score functions, $\mathbb{E}\{ l'_{\epsilon}(\bold{W} \lvert \bold{ \bar{W}};0) \lvert \bold{ \bar{W}} \} = 0$.

Our goal in this proof is to show that $\psi'_{\epsilon}(0) = \mathbb{E} \{\phi(\bold{Z}) l'_{\epsilon}(\bold{Z};0) \}$ for the proposed influence function 

$\phi(\bold{Z}) = (\mathbb{E} K_{bl}(\bold{X}))^{-1}
\{ \frac{Y-\mu(\bold{X},A)}{\pi(A\mid \bold{X})}w(A)K_{bl}(\bold{X}) + m(A) +  \int_{\mathscr{A}} [\mu(\bold{X},a)K_{bl}(\bold{X}) - m(a)]w(a)da \} - \psi$


First we give an expression for $\psi'_{\epsilon}(0)$.

By definition $\psi(\epsilon) = \int_{\mathscr{A}} \theta(a;\epsilon) w(a;\epsilon) da$, so 

$$  \psi'_{\epsilon}(0) =  
\int_{\mathscr{A}} 
\theta'_{\epsilon}(a;0) w(a)  + 
\theta(a) w'_{\epsilon}(a;0) da
= \mathbb{E} \{ \theta'_{\epsilon}(A;0) + \theta(A) w'_{\epsilon}(A;0)  \} $$


%% \epsilon

Also since $ \theta(a;\epsilon) =  \int_{\mathcal{X}} K_{bl}(\bold{x}) \mu(a,\bold{l}) d \upsilon(x) / \mathbb{E} K_{bl}( \bold{X}) = 
\int_{\mathcal{X}} K_{bl}(\bold{x}) \int_{\mathcal{Y}} yp(y\lvert \bold{x},a;\epsilon) d\eta(y) d \upsilon(x) /\mathbb{E} K_{bl}( \bold{X}) $





